Incremental Relational Lenses

Lenses are a popular approach to bidirectional transformations, a generalisation of the view update problem in databases, in which we wish to make changes to source tables to effect a desired change on a view. However, perhaps surprisingly, lenses have seldom actually been used to implement updatable views in databases. Bohannon, Pierce and Vaughan proposed an approach to updatable views called relational lenses, but to the best of our knowledge this proposal has not been implemented or evaluated to date. We propose incremental relational lenses, that equip relational lenses with change-propagating semantics that map small changes to the view to (potentially) small changes to the source tables. We also present a language-integrated implementation of relational lenses and a detailed experimental evaluation, showing orders of magnitude improvement over the non-incremental approach. Our work shows that relational lenses can be used to support expressive and efficient view updates at the language level, without relying on updatable view support from the underlying database.

==> fig/delta-relational-ops.tex <==
\begin{figure}
\begin{align*}
   \deltaselect{P}{M, \Delta M}
   &\defeq
   (\select{P}{\positive{\Delta M}}, \select{P}{\negative{\Delta M}})
   \\
   \deltaproj{M, \Delta M}{U}
   &\defeq
   (\proj{\positive{\Delta M}}{U} \setminus \proj{M}{U},
    \proj{\negative{\Delta M}}{U} \setminus \proj{M \deltaapp \Delta M}{U})
   \\
   (M, \Delta M) \deltaJoin (N, \Delta N)
   &\defeq
   (((M \deltaapp \Delta M) \Join \positive{\Delta N}) \cup (\positive{\Delta M} \Join (N \deltaapp \Delta N)),
    (\negative{\Delta M} \Join N) \cup (M \Join \negative{\Delta N}))
   \\
   \deltarename{A/B}{M, \Delta M}
   &\defeq
   (\rename{A/B}{\Delta M^+}, \rename{A/B}{\Delta M^-})
   \\
   (M, \Delta M) \deltacup (N, \Delta N)
   &\defeq
   (\positive{\Delta M} \cup \positive{\Delta N},
    (\negative{\Delta M} \setminus (N \deltaapp \Delta N)) \cup (\negative{\Delta N} \setminus (M \deltaapp \Delta M)))
   \\
   % (M, \Delta M) \deltacap (N, \Delta N)
   % &\defeq
   % (((\positive{\Delta M} \cap (N \deltaapp \Delta N)) \cup (\positive{\Delta N} \cap (M \deltaapp \Delta M)),
   %  \negative{\Delta M} \cup \negative{\Delta N})
   % \\
   (M, \Delta M) \deltasetminus (N, \Delta N)
   &\defeq
   ((\positive{\Delta M} \setminus (N \deltaapp \Delta N)) \cup (\negative{\Delta N} \cap (M \setminus \negative{\Delta M})),
    (\negative{\Delta M} \setminus N) \cup \positive{\Delta N})
\end{align*}
\caption{Delta-relational operations}
\label{fig:delta-relational-ops}
\end{figure}


==> obsolete.tex <==
\begin{lemma}
   \label{lem:delta_diff}
   Suppose $N \subseteq M$ and $N \deltaapp \Delta N \subseteq M \deltaapp
   \Delta M$. Then $(M \deltaapp \Delta M) \setminus (N \deltaapp \Delta N) = (M
   \setminus N) \deltaapp (\Delta M \deltaminus \Delta N)$.
\end{lemma}

\begin{lemma}
   \label{lem:delta_rel_merge}
   If $\relmerge{M}{F}{N} = M$ then $\relmerge{M}{F}{N \deltaapp \Delta N} = \relmerge{M}{F}{\positive{\Delta N}}$
\end{lemma}

\subsection{Select Lens}

\begin{align*}
   \deltaOp{put}_v(M, \Delta N) &= (M_0, \Delta M_0) \deltasetminus (N_\#, \Delta N_\#) \\
   \text{where} \\
   N &= \getOp_v(M)
   \\
	(M_0, \Delta M_0)
   &=
   \deltarelmerge{\deltaselect{\neg P}{M, \emptyset}} {F}{(N, \Delta N)}
   \\
	(N_\#, \Delta N_\#) &= \deltaselect{P}{M_0, \Delta M_0} \deltasetminus (N, \Delta N)
\end{align*}
%
%\begin{align*}
%	I(R) \deltaapp \Delta I(R) &= (M_0 \deltaapp \Delta M_0) \setminus (N_\# \deltaapp \Delta N_\#) \\
%	M_0 \deltaapp \Delta M_0 &= \relmerge{\select{\neg P}{I(R)}}{F}{J(S) \deltaapp \Delta J(S)} \\
%	N_\# \deltaapp \Delta N_\# &= \select{P}{M_0 \deltaapp \Delta M_0} \setminus (J(S) \deltaapp \Delta J(S))
%\end{align*}

Using the correct definition of the select lens, we can derive the incremental
version as follows.
%
\begin{align*}
	\Delta M &= \Delta M_0 \deltaminus \Delta N_\# \\
	\Delta M_0 &= \relmerge{\select{\neg P}{M}}{F}{\positive{\Delta N}} \deltaminus \select{\neg P}{M} \\
	\Delta N_\# &= \select{P}{\Delta M_0} \deltaminus \Delta N
\end{align*}

The definition of $\Delta M_0$ follows from
Lemma~\ref{lem:correctness-delta-ops} part (2) and
Lemma~\ref{lem:delta_rel_merge}.

We know that $N \deltaapp \Delta N \subseteq M_0 \deltaapp \Delta M_0$, and that
$N \deltaapp \Delta N \subseteq P$. This means that $N \deltaapp \Delta N
\subseteq \select{P}{M_0 \deltaapp \Delta M_0}$ since $\forall r \in N, r \in
M_0 \deltaapp \Delta M_0 \wedge r \in P$. This allows us to apply
Lemma~\ref{lem:delta_diff} to derive $\Delta N_\#$.

We know that $N_\#$ is a subset of $M_0$, since it is calculated using the
intersection of $M_0$ minus a further set. This along with
Lemma~\ref{lem:delta_diff} allow us to derive the definition of $\Delta M$.

\subsection{Join lens}

\begin{align*}
   \deltaOp{put}(\Delta O, (M, N)) &= ((M', \Delta M'), (N', \Delta N')) \\
   \text{where} \\
   O &= \getOp(M, N) \\
   (M_0, \Delta M_0) &= \Delta{\relmerge{(M, \emptyset)}{F}{\deltaproj{O, \Delta O}{U}}} \\
	(N_0, \Delta N_0) &= \Delta{\relmerge{(N, \emptyset)}{G}{\deltaproj{O, \Delta O}{V}}} \\
	(L, \Delta L) &= ((M_0, \Delta M_0) \deltaJoin (N_0, \Delta N_0)) \deltasetminus (O, \Delta O) \\
	(L_l, \Delta L_l) &= (L, \Delta L) \deltaJoin \deltaproj{O, \Delta O}{U \cap V} \\
	(L_a, \Delta L_a) &= (L, \Delta L) \deltasetminus (L_l, \Delta L_l) \\
	(M', \Delta M') &= ((M_0, \Delta M_0) \deltasetminus \deltaproj{\deltaselect{P_d}{L_a, \Delta L_a}}{U}) \deltasetminus \deltaproj{L_l, \Delta L_l}{U} \\
	(N', \Delta N') &= (N_0, \Delta N_0) \deltasetminus \deltaproj{\deltaselect{\smash{P_d}'}{L_a, \Delta L_a}}{V}
\end{align*}

Note: $(A \Join \proj{B}{X}) \deltaapp (A \Join \Delta \proj{B}{X})$ is not
necessarily the same as $A \Join \proj{B \deltaapp \Delta B}{X}$. This is because
projections get rid of multiplicity and so may have ill consequences. The
solution is to perform the join first and then only the projection.

These definitions are simplified by the fact that we know $L$, $L_l$ and $L_a$
must be $\emptyset$, because no rows are deleted if the output table contains no
changes. Thus $\Delta L = L \deltaapp \Delta L$ and the same applies to $L_l$ and
$L_a$.

The two subsets $\Delta M_0$ and $\Delta N_0$ can be calculated using the
methods described in Section \ref{section:querying_rel_merge}. Calculating
$\Delta L$ requires two further queries to be able to calculate $\Delta M_0
\Join N_0$ and $\Delta N_0 \Join M_0$. These can be found calculated by querying
for $\sigma_{U \cap V \in \proj{\Delta M_0}{U \cap V}}(N)$ and $\sigma_{U \cap V
\in \proj{\Delta N_0}{U \cap V}}(M)$.

Finally we need to query a small subset of the database in order to be able to
determine what $\Delta L \Join \proj{J(T)}{U \cap V}$ should be in order to be
able to calculate $L_l$. This can be done by querying for $\proj{\sigma_{U \cap
V \in \proj{\Delta L}{U \cap V}}(M \Join N)}{U \cap V}$.

% \section{Join template}

% \jrcnote{TODO: State join template definition and typing rule.  Show
%   how to define the other variants of joins in terms of it.}

% \citet{bohannon2006relational} define several lenses associated with
% join, preferring to delete from the left, right or both sources when a
% tuple in the view is deleted.  They also show that all three can be
% defined as instances of a \emph{join template} lens that can also be
% instantiated in other ways.  Essentially, the idea is to parameterise
% the join template lens with predicates $P_d$ and $P_d'$ such that
% a tuple is deleted from the left source table if $P_d$ holds, from the
% right source table if $P_d'$ holds, and from both tables if both
% hold.  Thus, for well-behavedness it is necessary to check that at
% least one of these predicates holds for any possible view tuple,
% according to the following typing rule:
% \[
%    \inferrule*[right={T-Join}]
%         {
%         	\label{eq:t_join}
%         	G \vDash U \cap V \to V
%         	\\
%         	P_d \vee Q_d = \top_{UV}
%         	\\
%         	P\text{ ignores }\outputs(F)
%         	\\
%         	Q\text{ ignores }\outputs(G)
%         }
%         {
%         	\JoinPrim{P_d}{Q_d}:
%       \vtype{U}{P}{F} \otimes \vtype{V}{P'}{G} \lensto \vtype{U \cup V}{P \Join Q}{F \cup G}
%         }
% \]


% The lens $\JoinPrim{P_d}{Q_d}: \vtype{U}{P}{F} \otimes \vtype{V}{Q}{G}
% \lensto \vtype{ U\cup V}{P \Join Q}{ F \cup G}$ is given by the functions $\getOp$
% and $\putOp$ defined as follows:
% %
% \[\begin{array}{lrcl}
% &	\getOp(M,N) &=& M \Join N
% 	\\
% &	\putOp((M,N), O) &=& \letexpr{M_0}{\relmerge{M}{F}{\proj{O}{U}}}{}
% 	\\
% &&&\letexpr{N_0 }{ \relmerge{N}{G}{\proj{O}{V}}}{}
% 	\\
% &&&\letexpr{	L }{ (M_0 \Join N_0) \setminus O}{}
% 	\\
% &&&\letexpr{	L_l }{ L \Join \proj{O}{U \cap V}}{}
% 	\\
% &&&\letexpr{	L_a }{ L \setminus L_l}{}
% 	\\
% &&&\letexpr{	M' }{ (M_0 \setminus \proj{\select{P_d}{L_a}}{U}) \setminus \proj{L_l}{U}}{}
% 	\\
% &&&\letexpr{	N' }{ N_0 \setminus \proj{\select{Q_d}{L_a}}{V}}{}
% \\
% &&& (M',N')
% \end{array}\]

% \jrcnote{TODO discuss and explain how the left right and both primitives can be
% defined as special cases.}


% \jrcnote{TODO: Give delta version of join template?}

\subsection{Additional optimisations}
\label{section:additional_optimisations}

In the incremental definition of projection, the value of $\Delta M$ only
depends on certain parts of $M$, and so it can be calculated more efficiently
using the following. Note that the relational merge operation normally requires
the two relations to have the same domain, but ignoring the mismatch still
produces the correct result.
%
\[
	\relmerge{\Delta M'}{X \to A}{\select{X \in \proj{M}{X}}{M}}
\]

Most lenses require the relational merge operation, which takes merges in a set
$N$ into another set $M$ while performing any functional updates. For every
record in $N$ and functional dependency $X \to Y$, the operation updates all
records in $M$ which have the same value for $X$ as some record in $N$ so that
they have the same value for $Y$.
%
\begin{equation}
	\label{eq:rel_merge}
	M_0 = \relmerge{M}{F}{\positive{\Delta N}} \\
\end{equation}

Given that we are only interested in the change set, we can calculate $\Delta
M_0$ by subtracting the set $M$ after the operation as shown in Equation
\ref{eq:delta_relmerge_inefficient}. The naive version of calculating the output
$\Delta M_0$ requires the entire table $M$ to be queried. To avoid the high cost
of calculating $\Delta M_0$ we need a method that doesn't rely on the entire
table $M$.
%
\begin{equation}
   \label{eq:delta_relmerge_inefficient}
	\Delta M_0 = \relmerge{M}{F}{\positive{\Delta N}} \deltaminus M
\end{equation}

We know that any record in $M$ which is not changed by $\positive{\Delta N}$
will be removed by the subtraction of $M$ after the update. It is not necessary
to perform the relational merge operation on the entire set of $M$, but only the
subset which will change. The solution is to formulate a query $P$, which will
query the database for those records which are likely to be affected by the
delta.

We define $\affected$ as
\[ \affected_F(N) \defeq \bigvee_{X \to Y \in F} X \in \proj{N}{X}. \]

An example of $P=\opname{affected}_F(N)$ for the example update set shown in
Figure \ref{ex:updateset} would be \[ P = A \in \set{1, 2, 4} \vee B \in \set{1,
3, 5} \]

Theorem \ref{thm:delta_rel_merge_two} shows that it is possible to replace $M$
in Equation \ref{eq:rel_merge} with $\select{P}{M}$, where $P =
\opname{affected}_F(N)$ so that our query becomes \[ \Delta M_0 =
\relmerge{\select{P}{M}}{F}{\positive{\Delta N}} \deltaminus \select{P}{M}. \]

% \subsection{Update Set}

% 	Another way to describe the functional updates is through an update set. An
% 	update set contains the mappings of values for each functional dependency $f$
% 	in a set of functional dependencies $F$. Example \eqref{ex:updateset} shows
% 	the update set of a given change set $\Delta R$.

% 	\begin{align}
% 		\label{ex:updateset}
% 		\begin{array}{c|ccc}
% 			\Delta R & A & B & C \\
% 			\hline
% 			-1 & 1 & 2 & 3 \\
% 			+1 & 1 & 3 & 2 \\
% 			-1 & 2 & 1& 3 \\
% 			+1 & 2 & 1 & 4 \\
% 			+1 & 4 & 5 & 6 \\
% 			-1 & 5 & 6 & 7
% 		\end{array}
% 		\quad\implies\quad
% 		\begin{array}{l}
% 			A \to B: \\
% 			\qquad 1 \to 3 \\
% 			\qquad 2 \to 1 \\
% 			\qquad 4 \to 5 \\
% 			\\
% 			B \to C: \\
% 			\qquad 1 \to 4 \\
% 			\qquad 3 \to 2 \\
% 			\qquad 5 \to 6
% 		\end{array}
% 	\end{align}

% 	The definition of $\opname{get\_fd\_updates}$ is used, which takes a change set $\Delta R$ as well as a functional
% 	dependency $X \to Y$ and determines all new mappings from $\Left(X \to Y)$ to $\Right(X\to Y)$. It does this by
% 	finding all changes in the change set $\Delta R$ where the multiplicity is $+1$ and then projects them onto
% 	$\Left(X \to Y)$ and $\Right(X \to Y)$.

% 	% \begin{align*}
% 	%	& \defn{get\_fd\_updates} \argDR\ (f : \type{fundep}) := \\
% 	%	& \qquad \left( f, \left\{ \pi_{\Left(fd)}(t), \pi_{\Right(fd)}(t) \mid (t,+1) \in \Delta R \right\} \right)
% 	% \end{align*}

% 	Using $\opname{get\_fd\_updates}$, $\opname{get\_updateset}$ is defined which takes a change set $\Delta R$ as well
% 	as the set of functional dependencies $F$ and calculates the set of $\opname{get\_fd\_updates}$ for each functional
% 	dependency $f$ in $F$.

% 	% \begin{align*}
% 	%	& \defn{get\_updateset} \argDR\ (F : \type{fundepset}) := \\
% 	%	& \qquad \left\{ \opname{get\_fd\_updates} \Delta R\ f \mid f \in F \right\}
% 	% \end{align*}

\iffalse
We produce a table where every entry can either be '+', '-' or ' ' signalling that a row $m$ is either present, negatively present or not present at all. We iterate through all posibilities within a table as shown below. If one of the following conditions are violated, we don't calculate the result, and if none of them are violated the results need to match up:

\begin{enumerate}
		\item $N \subseteq M$
		\item $(N \deltaplus \Delta N) \subseteq (M \deltaplus \Delta M)$
		\item $N, \Delta N$ minimal
		\item $M, \Delta M$ minimal
\end{enumerate}

\begin{longtable}{cccc|cc|c}
$\in M$ & $\in \Delta M$ & $\in N$ & $\in \Delta N$ & $(M \deltaplus \Delta M) \setminus (N \deltaplus \Delta N)$ & $(M \setminus N) \deltaplus (\Delta M \deltaminus \Delta N)$ & violates \\
\hline
  &   &   &   &  &   & \\
  &   &   & + && & (2) \\
  &   &   & - && & (2) \\
  &   & + &   && & (1, 2) \\
  &   & + & + && & (1, 2, 3) \\
  &   & + & - && & (1) \\
  & + &   &   &+ & + & \\
  & + &   & + &  &   & \\
  & + &   & - && & (2) \\
  & + & + &   && & (1) \\
  & + & + & + && & (1, 3) \\
  & + & + & - && & (1) \\
  & - &   &   &- & - & \\
  & - &   & + && & (2) \\
  & - &   & - &  &   & \\
  & - & + &   && & (1, 2) \\
  & - & + & + && & (1, 2, 3) \\
  & - & + & - && & (1) \\
+ &   &   &   &+ & + & \\
+ &   &   & + &  &   & \\
+ &   &   & - && & (2) \\
+ &   & + &   &  &   & \\
+ &   & + & + && & (3) \\
+ &   & + & - &+ & + & \\
+ & + &   &   && & (4) \\
+ & + &   & + && & (4) \\
+ & + &   & - && & (2, 4) \\
+ & + & + &   && & (4) \\
+ & + & + & + && & (3, 4) \\
+ & + & + & - && & (4) \\
+ & - &   &   &  &   & \\
+ & - &   & + && & (2) \\
+ & - &   & - && & (2) \\
+ & - & + &   && & (2) \\
+ & - & + & + && & (2, 3) \\
+ & - & + & - &  &   & \\
\end{longtable}
\fi

\iffalse
	% We don't need this lemma because of our new general record revision operator
\begin{lemma}
	If $\recrevise{m}{B \deltaapp \Delta B}{X \to Y}{m'}$ and
	$\recrevise{m}{\positive{\Delta B}}{X \to Y}{m''}$ then $m' = m''$ if $m \in B$.
\end{lemma}

\begin{proof}

	We assume that $B \deltaapp \Delta B = (B \setminus \negative{\Delta B}) \cup
	\positive{\Delta B}$. Suppose there exists $n \in B \setminus
	\negative{\Delta B}$ such that $\recproj{m}{X} = \recproj{n}{X}$. Then we
	know that $\proj{m}{Y} = \recproj{n}{Y}$, since $B \vDash X \to Y$ and $B
	\subseteq B \deltaapp \Delta B$. There cannot be a $n' \in \positive{\Delta
	B}$ with $\recproj{n'}{X} = \recproj{n}{X} \wedge \recproj{n'}{Y} \neq
	\recproj{n}{Y}$, since this would violate $B \deltaapp \Delta B \vDash X \to Y$.
	If we apply the rule \eqref{eqn:c-match} to the case $\recrevise{m}{B \deltaapp
	\Delta B}{X \to Y}{m'}$ then $m' = \recupdate{m}{\recproj{n}{Y}} = m$. In the
	case of $\recrevise{m}{\positive{\Delta B}}{X \to Y}{m''}$ if there exists a
	record $n' \in \positive{\Delta B}$ so that $\recproj{n'}{X} =
	\recproj{n}{X}$ then we apply \eqref{eqn:c-match} and $m'' =
	\recupdate{m}{\recproj{n}{Y}} = m$, otherwise we apply \eqref{eqn:c-nomatch}
	and $m'' = m$. Thus we have $m' = m'' = m$.

	If no such $n$ exists in $B \cup \negative{\Delta B}$, then it depends on if
	there exists a record $n' \in \positive{\Delta B}$. If there isn't then we
	apply \eqref{eqn:c-nomatch} to both cases and $m' = m'' = m$. If there is,
	then $m' = \recupdate{m}{\recproj{n'}{Y}}$ and $m'' =
	\recupdate{m}{\recproj{n'}{Y}}$ and so $m' = m'' =
	\recupdate{m}{\recproj{n'}{Y}}$.
\end{proof}
\fi

\iffalse
	% Don't need this anymore because our recrevise skips this
	\begin{lemma}
		\label{lemma:record_revision}
		% We assume $m : U$, $N : U$, $X \to Y : U$, $N \vDash X \to Y$, $X \to Y \in F$ and $P = \affected(F, N)$.
		If $m \notin \select{P}{N}$, then $\recrevise{m}{N}{X \to Y}{m'}$ implies $m' = m$.
	\end{lemma}

	\begin{proof}
		We know that $m \notin \select{P}{N}$ since $\recproj{m}{X} \notin \proj{N}{X}$.
		This means that \eqref{eqn:c-nomatch} is applied for every such $m$ and so $m' = m$.
	\end{proof}
\fi

